Analysis of diversity-accuracy tradeoff in image captioning

We investigate the effect of different model architectures, training objectives, hyperparameter settings and decoding procedures on the diversity of automatically generated image captions. Our results show that 1) simple decoding by naive sampling, coupled with low temperature is a competitive and fast method to produce diverse and accurate caption sets; 2) training with CIDEr-based reward using Reinforcement learning harms the diversity properties of the resulting generator, which cannot be mitigated by manipulating decoding parameters. In addition, we propose a new metric AllSPICE for evaluating both accuracy and diversity of a set of captions by a single value.

==> sections/bg.tex <==
\section{Related work}
\rtcom{Many are copied. Need to paraphrase.}

\rtcom{
\cite{batra2012diverse} formalized this task for Markov Random Fields as the DivMBest problem and presented a greedy approach which solves for outputs iteratively, conditioning on previous solutions to induce diversity.\\
\cite{gimpel2013systematic} apply DivMBest to machine translation using beam search as a black-box inference algorithm.
}

\rtcom{
\cite{vijayakumar2016diverse} provides a simple way to generate diverse sets. They experiement with different B and G and $\lambda$s; they also experiment what kind of suppression to use and in the end hamming distance works the best. They mostly evaluate on oracle-score and Distinct bigram ratio; they also did humen expreiments (group=1 vs group=6).
}
\rtcom{
Efforts have been made by \cite{li2015diversity} and \cite{li2016mutual} to produce diverse decodings from recurrent models for conversation modeling and machine translation by introducing novel heuristics
within the Beam Search (BS) algorithm.\\
\cite{li2016mutual} proposes a BS diversification
heuristic that discourages beams from sharing common
roots, implicitly resulting in diverse lists.
\cite{li2015diversity} introduce a novel decoding
objective that maximizes mutual information between inputs and predictions to penalize generic sequences.
}


\rtcom{
\cite{jain2017creativity} proposes a vae model for generating diverse visual questions. \cite{wang2017diverse}
proposes to use a stronger prior distribution instead a single guassian.
}

\rtcom{
\cite{shetty2017speaking, dai2017towards} proposes using gans. 
}

\rtcom{
\cite{wang2016diverse} grouptalk train 3 models sequentially in a adaboost-like way.
\cite{shen2019mixture} propose a mixture of experts model for machine translation task and found it can outperform diverse beam search.
}

\cite{chen2018groupcap} generates diverse captions for a group of images.

\rtcom{
\cite{fan2018hierarchical, radford2019language} use topk sampling.
\cite{Ari2019nucleus} studies the reason of repetition in beam search and bad sampling result in random sampling, and propose nucleus sampling.
}

\rtcom{
\cite{deshpande2018diverse} proposes a hierachical (POS-tag to word) method to enforce diversity in POS-tagging of potential words. (\rtcom{need to be compared} I want to but we can't. I don't really feel like their conclusion is correct about diversity. I feel like dbs is really really diverse. They are using non-standard split(why??!!!!))
}

\rtcom{
The most relevant work to ours is \cite{wang2019describing}. They proposed a new diversity metric self cider. They also did a complete survey on SOTA models on diversity. They found jointly training with cider reward and cross entropy loss can balance between diversity and accuracy. However, they mostly investigate random sampling only under temperature 1. In fact, different sampling temperature can get us results with different level of diversity from one single model.\\
In addition to that, other sophisticated sampling method like topk sampling, nucleus sampling and diverse beam search are not investigated. One of the conclusion of their paper is that model trained with cross entropy loss have high diversity but low accuracy when doing random sampling. This is a common finding that random sampling leads to bad results, and recently necleus sampling paper analyzed this phenomenon. A better way to use random sampling is to consider these variants like topk sampling and nucleus sampling.
}

\section{Conclusion}
